Cn2 profile from Shack-Hartmann data with CO-SLIDAR data processing

Cn2 profile monitoring usually makes use of wavefront slope correlations or of scintillation pattern correlations. Wavefront slope correlations provide sensitivity to layers close to the receiving plane. In addition, scintillation correlations allow a better sensitivity to high turbulence layers. Wavefront slope and scintillation correlations are therefore complementary. Slopes and scintillation being recorded simultaneously with a Shack-Hartmann wavefront sensor (SHWFS), we propose here to exploit their correlation to retrieve the Cn2 profile. The measurement method named COupled SLodar scIDAR (CO-SLIDAR) uses correlations of SHWFS data from two separated stars. A maximum-likelihood method is developed to estimate precisely the positions and intensities corresponding to each SHWFS spot, which are used as inputs for CO-SLIDAR. First results are presented using SHWFS real data from a binary star.

==> m-ch-en.tex <==
% name      : PPCHTEX / english interface
% version   : 1997.03.05
% author    : J. Hagen
% copyright : J. Hagen, A.F. Otten

\chardef\interfacenumber=0

\input ppchtex.noc

\endinput


==> m-pictex.tex <==
%D \module
%D   [       file=m-pictex,
%D        version=1997.01.15,
%D          title=\CONTEXT\ Extra Modules,
%D       subtitle=\PICTEX\ Loading Macros,
%D         author=Hans Hagen,
%D           date=\currentdate,
%D      copyright={PRAGMA / Hans Hagen \& Ton Otten}]
%C
%C This module is part of the \CONTEXT\ macro||package and is
%C therefore copyrighted by \PRAGMA. See mreadme.pdf for
%C details.

%D This module is one big hack. This hack is not needed when
%D using \ETEX, so there we simply load \PICTEX\ and quit.

%D Not every package defines \type{\fiverm}, \PICTEX's pixel,
%D so let's take care of that omision here. The actual loading
%D of \PICTEX\ depends on the package. For \LATEX\ users we
%D take care of loading the auxiliary ones too.

\def\loadpictex
  {\ifx\grid\undefined \else \let\normalgrid\grid \fi
   \ifx\axis\undefined \else \let\normalaxis\axis \fi
   \ifx\undefined\fiverm
     \font\fiverm=cmr5
   \fi
   \ifx\beginpicture\undefined
     \ifx\newenvironment\undefined
       \readfile{thrd-pic.tex}{}{}
     \else
       \input prepictex.tex  \relax
       \input pictex.tex     \relax
       \input postpictex.tex \relax
     \fi
   \fi
   \ifx\normalgrid\undefined \else
     \let\pictexgrid\grid
     \let\grid\normalgrid
   \fi
   \ifx\normalaxis\undefined \else
     \let\pictexaxis\axis
     \let\axis\normalaxis
   \fi}

\ifx\eTeXversion\undefined \else \loadpictex \expandafter \endinput \fi

%D When not in \ETEX\ and not in \CONTEXT, we load a few
%D auxiliary macros.

\ifx \undefined \writestatus \input supp-mis.tex \relax \fi

\unprotect

%D \TEX\ provides 256 \DIMENSIONS\ and 256 \SKIPS. In \CONTEXT\
%D this is no problem, but in packages that have many
%D authors, one can be quite sure that a lot of \DIMENSIONS\ are
%D allocated. Packages that use \PICTEX\ can therefore run out
%D of \DIMENSIONS\ quite fast. This module was written as a
%D reaction to persistent problems with loading \PPCHTEX\ in
%D \LATEX\ and \PICTEX\ deserves a solution. I therefore
%D dedicate this module to Tobias Burnus and Dirk Kuypers, who
%D use \PPCHTEX\ in a \LATEX\ environment and suggested a lot
%D of extensions to the repertoire of \PPCHTEX\ commands.
%D
%D This module presents a solution that is quite effective: all
%D \DIMENSIONS\ are drawn from the pool of \DIMENSIONS\ and
%D \SKIPS, depending on the availability. This is possible
%D because \DIMENSIONS\ are \SKIPS\ without a glue component.
%D Therefore we can use \SKIPS\ as \DIMENSIONS. However, some
%D incompatibility can result from assignments that look like:
%D
%D \starttyping
%D \somedimen=\someskip
%D \stoptyping
%D
%D In such cases the \DIMENSION\ equals the fixed part of the
%D \SKIP\ or in other words: this assignment strips off the
%D glue. Because \PICTEX\ uses no glue components, I thought
%D I could interchange both register types without problems,
%D but alas, this didn't hold for all \DIMENSIONS.

%D In \PLAIN\ \TEX\ the allocation macros are defined with (as)
%D \type{\outer}. This means that they cannot appear inside
%D macros, not even in an indirect way. We therefore have to
%D redefine both \type{\newdimen} and \type{\newskip} to
%D non||\type{\outer} alternatives. In most macro packages this
%D redefinition already took place. We save the original
%D meanings, so we can restores them afterwards.

% \def\temporarynewdimen {\alloc@1\dimen\dimendef\insc@unt}
% \def\temporarynewskip  {\alloc@2\skip \skipdef \insc@unt}

\let\normalnewdimen   \newdimen
\let\normalnewskip    \newskip

\let\temporarynewdimen\newdimen
\let\temporarynewskip \newskip

%D Here comes the trick. Depending on how many \DIMENSIONS\ and
%D \SKIPS\ are allocated, the \type{\newdimen} assigns a
%D \DIMENSIONS\ or \SKIP. \PLAIN\ \TEX\ allocates 15 \DIMENSIONS\
%D and 17 \SKIPS. After loading \PICTEX, 71 \DIMENSIONS\ and
%D and 71 \SKIPS\ are allocated. Indeed, \PICTEX\ needs 110
%D \DIMENSIONS !
%D
%D \starttyping
%D \def\newdimen
%D   {\ifnum\count11>\count12
%D      \let\next\temporarynewskip
%D    \else
%D      \let\next\temporarynewdimen
%D    \fi
%D    \next}
%D \stoptyping
%D
%D When I was testing a new version of \PPCHTEX\ in \PLAIN\
%D \TEX\ I had to find out that this exchange of registers
%D sometimes leads to unwanted results. It took me some hours
%D to find out that the source of errors originated in
%D constructions like:
%D
%D \starttyping
%D \ifdim\DimenOne<\DimenTwo whatever you want \else or not \fi
%D \stoptyping
%D
%D When \type{\DimenOne} is a \SKIP\ and \type{\DimenTwo} is a
%D \DIMENSION, \TEX\ scans for some optional glue component,
%D like in:
%D
%D \starttyping
%D \skip0=\dimen0 plus 10pt minus 5pt
%D \stoptyping
%D
%D The most robust solution to this problem is:
%D
%D \starttyping
%D \ifdim\DimenOne<\DimenTwo\relax right \else wrong \fi
%D \stoptyping
%D
%D Some close reading of the \PICTEX\ source however learned me
%D that this problem could be solved best by just honoring the
%D allocation of \DIMENSIONS\ when the name of the macro
%D explictly stated the character sequence \type{dimen}. A next
%D implementation therefore automatically declared all
%D \DIMENSIONS\ with this sequence in their names with
%D \type{\dimen}. Again I was too optimistic, so now we do it
%D this way (the comments are from \PICTEX, which like \TABLE,
%D is an example of a well documented package):

\temporarynewdimen\!dimenA       %.AW.X.DVEUL..OYQRST
\temporarynewdimen\!dimenB       %....X.DVEU...O.QRS.
\temporarynewdimen\!dimenC       %..W.X.DVEU......RS.
\temporarynewdimen\!dimenD       %..W.X.DVEU....Y.RS.
\temporarynewdimen\!dimenE       %..W........G..YQ.S.
\temporarynewdimen\!dimenF       %...........G..YQ.S.
\temporarynewdimen\!dimenG       %...........G..YQ.S.
\temporarynewdimen\!dimenH       %...........G..Y..S.
\temporarynewdimen\!dimenI       %...BX.........Y....
\temporarynewdimen\!dxpos        %..W......U..P....S.
\temporarynewdimen\!dypos        %..WB.....U..P......
\temporarynewdimen\!xloc         %..WB.....U.......S.
\temporarynewdimen\!xpos         %..........L.P..Q.ST
\temporarynewdimen\!yloc         %..WB.....U.......S.
\temporarynewdimen\!ypos         %..........L.P..Q.ST
\temporarynewdimen\!zpt          %.AWBX.DVEULGP.YQ.ST

%D Tobias tested this module in all kind of \LATEX\ dialects
%D so we were able to find out that we also needed to declare:

\temporarynewdimen\linethickness

%D After all, the new definition of \type{\newdimen} became:

\def\newdimen#1%
  {\ifx#1\undefined
     \ifnum\count11>\count12\relax
       \temporarynewskip#1\relax
     \else
       \temporarynewdimen#1\relax
     \fi
     %\edef\ascii{\meaning#1}%
     %\immediate\write20{\string#1 becomes \ascii}%
   \else
     %\edef\ascii{\meaning#1}%
     %\immediate\write20{\string#1 already is \ascii}%
   \fi}

% \def\newdimen#1%
%   {\bgroup
%    \escapechar=-1
%    \def\next##1##2%
%      {\def\next####1##1####2####3\next%
%         {\egroup
%          \if####2@
%            \temporarynewdimen#1\relax
%          \ifnum\count11>\count12
%            \temporarynewskip#1\relax
%          \else
%            \temporarynewdimen#1\relax
%          \fi\fi}%
%       \expandafter\next\string##2##1@@\next}%
%    \expandafter\next\expandafter{\string\dimen}#1}
%
% This macro is as unreadable, inefficient and as compact as
% can be, but uses no extra hash entries, which sometimes are
% scarce too. A more readable alternative, that also takes
% explicit \SKIPS\ into account, is included in the source.
%
% \def\doifregisterpreferenceelse#1#2#3#4%
%   {\def\dodoifregisterpreferenceelse##1#1##2##3\war{\if##2@}%
%    \expandafter\dodoifregisterpreferenceelse\string#2#1@@\war
%      #4%
%    \else
%      #3%
%    \fi}
%
% \def\newdimen#1%
%   {\bgroup
%    \escapechar=-1
%    \expandafter\doifregisterpreferenceelse\expandafter{\string\dimen}#1
%      {\egroup
%       \temporarynewdimen#1}
%      {\expandafter\doifregisterpreferenceelse\expandafter{\string\skip}#1
%         {\egroup
%          \temporarynewskip#1}
%         {\egroup
%          \ifnum\count11>\count12
%            \temporarynewskip#1\relax
%          \else
%            \temporarynewdimen#1\relax
%          \fi}}}

%D Curious readers can still find the previous solution in
%D the source. The next macro is used instead of
%D \type{\input}. This macro also reports some statistics.

\def\dimeninput#1 %
  {\message{[before: d=\the\count11,s=\the\count12]}%
   \input #1 \relax
   \message{[after: d=\the\count11,s=\the\count12]}}%

%D Now we can load \PICTEX:

\loadpictex

%D Finally we restore the old definitions of \type{\newdimen}
%D and \type{\newskip}:

\let\newdimen=\normalnewdimen
\let\newskip =\normalnewskip

%D and just hope for the best.

\protect \endinput

